SGL: Symbolic Goal Learning in a Hybrid, Modular Framework for Human Instruction Following

This paper investigates robot manipulation based on human instruction with ambiguous requests. The intent is to compensate for imperfect natural language via visual observations. Early symbolic methods, based on manually defined symbols, built modular framework consist of semantic parsing and task planning for producing sequences of actions from natural language requests. Modern connectionist methods employ deep neural networks to automatically learn visual and linguistic features and map to a sequence of low-level actions, in an endto-end fashion. These two approaches are blended to create a hybrid, modular framework: it formulates instruction following as symbolic goal learning via deep neural networks followed by task planning via symbolic planners. Connectionist and symbolic modules are bridged with Planning Domain Definition Language. The vision-and-language learning network predicts its goal representation, which is sent to a planner for producing a task-completing action sequence. For improving the flexibility of natural language, we further incorporate implicit human intents with explicit human instructions. To learn generic features for vision and language, we propose to separately pretrain vision and language encoders on scene graph parsing and semantic textual similarity tasks. Benchmarking evaluates the impacts of different components of, or options for, the vision-and-language learning model and shows the effectiveness of pretraining strategies. Manipulation experiments conducted in the simulator AI2THOR show the robustness of the framework to novel scenarios.

==> discussion.tex <==
\section{Discussion}
\subsection{Classification v.s. Regression}
One of the major differences between this work and previous approaches is to classify grasp angles into different categories, rather than directly regress to a single angle. This trick is based on the fact that CNNs are known to perform better classification task than regression task. Our experiments also shows that classification results indeed reflects the orientation of grasp, whereas the regressed angles tend to be erroneous. One drawback of regression based approach is that, the output usually regresses to the center of potential grasp due to averaging effect as in Fig. \ref{fig_case_not_averaged}. Also, regressed location is easily off the desired grasp. Fig. \ref{fig_case_failure_original} shows some failure cases of regression based approach. One other benefit of doing classification on candidate regions is that we can thus avoid manipulating rotated feature maps between network layers, which may potentially cause error due to the size of feature maps is typically small close to the output.  



\subsection{What objects are missing?}
One can observe that although we achieve high precision rate, the recall rate shows that we are unable to detect grasps one some objects. Before we investigate further, note that regression based approach always produces a predicted region, while our approach only predict one or more grasps when the system is confidential. Hence, the recall rate for previous approach is 100\% whereas ours is lower. Now, once a candidate region is produced by our system, we require the highest softmax score among all classes is above the threshold(0.8 in this work). And the system assigns class label representing the orientation of grasp to the candidate region. This might cause problem in two cases. The first case is when the object is round shape. And the second case is when the object is too small in the input image. Two cases cause the system find it hard to decide which orientation to assign, and the softmax scores for each class are equally small and below threshold. We output the images with missing grasp in Fig. \ref{fig_case_not_detected}. and it confirms our guess.















%\begin{figure}[t]
%    \centering
%    \includegraphics[width=2.8in]{fig_case_failure_original}
%    \caption{Failure cases of \cite{redmon2015real}. Regression tends to shift %from objects and causes invalid predictions.}
%    \label{fig_case_failure_original}
%\end{figure}

  

\begin{figure}[t]
    \centering
    \includegraphics[width=3.4in]{fig_case_not_detected}
    \caption{Failure cases using classification instead of regression. Round-shape like objects and tiny objects may have similar scores across all types of grasp, resulting in none of them has score above threshold, and thus no predicted grasps.}
    \label{fig_case_not_detected}
\end{figure}





\subsection{Multiple Grasps}
Our work is able to predict multiple grasp candidates without using sliding windows or dividing original input image into several grid. Hence the processing time is fast and the position of possible grasps is not limited to the grid cell. With more high quality grasps predicted, this system provides options for users to select most appropriate grasp to manipulate object. For example, one can choose the closest grasp, or choose grasp based on the functionality or the purpose of robot.      


\subsection{Pre-trained networks}
We chose to replace one of the original RGB channel with depth data in order to re-use pre-trained weights. A good pre-trained network is greatly helpful to quickly converge to better local minima point other than stuck in bad local minima. In our case the pre-trained weights originally for RGB seem to also work nicely for RGD data. By using VGG trained on ImageNet, this architecture is able to learn meaningful region proposal, regression and classification. Multiple grasp candidates can be predicted for novel objects.    



